Sparse Tensor Algebra Optimizations with Workspaces

This paper shows how to optimize sparse tensor algebraic expressions by introducing temporary tensors, called workspaces, into the resulting loop nests. We develop a new intermediate language for tensor operations called concrete index notation that extends tensor index notation. Concrete index notation expresses when and where sub-computations occur and what tensor they are stored into. We then describe the workspace optimization in this language, and how to compile it to sparse code by building on prior work in the literature. We demonstrate the importance of the optimization on several important sparse tensor kernels, including sparse matrix-matrix multiplication (SpMM), sparse tensor addition (SpAdd), and the matricized tensor times Khatri-Rao product (MTTKRP) used to factorize tensors. Our results show improvements over prior work on tensor algebra compilation and brings the performance of these kernels on par with state-of-the-art hand-optimized implementations. For example, SpMM was not supported by prior tensor algebra compilers, the performance of MTTKRP on the nell-2 data set improves by 35%, and MTTKRP can for the first time have sparse results.

==> Makefile <==
pdf: paper.pdf
.PHONY: pdf

paper.pdf: 
	latexmk -pdf paper.tex
.PHONY: paper.pdf

notodo:
	latexmk -pdf -pdflatex='pdflatex %O -interaction=nonstopmode -synctex=1 "\def\notodo{1}\input{%S}"'paper.tex
.PHONY: notodo

paper.ps: paper.pdf
	acroread -toPostScript $<

clean:
	latexmk -C paper.tex
	rm -f *.bbl *.log
.PHONY: clean

view: paper.pdf
	open paper.pdf
.PHONY: view

safe: paper.pdf
	mkdir -p archive
	cp $^ archive/`date "+%y.%m.%d-%H.%M.%S"`-`openssl md5 < $^`.pdf


